Towards Automated Circuit Discovery for Mechanistic Interpretability

Through considerable effort and intuition, several recent works have reverse-engineered nontrivial behaviors of transformer models. This paper systematizes the mechanistic interpretability process they followed. First, researchers choose a metric and dataset that elicit the desired model behavior. Then, they apply activation patching to find which abstract neural network units are involved in the behavior. By varying the dataset, metric, and units under investigation, researchers can understand the functionality of each component. We automate one of the process' steps: to identify the circuit that implements the specified behavior in the model's computational graph. We propose several algorithms and reproduce previous interpretability results to validate them. For example, the ACDC algorithm rediscovered 5/5 of the component types in a circuit in GPT-2 Small that computes the Greater-Than operation. ACDC selected 68 of the 32,000 edges in GPT-2 Small, all of which were manually found by previous work. Our code is available at https://github.com/ArthurConmy/Automatic-Circuit-Discovery.

==> archive/intro_save.tex <==
\section{Introduction}

One aim of interpretability in machine learning is to explain model outputs in terms of the internal components of that model \citep{zhang2021survey}. 
In prior work, \citet{olah2020zoom} explain curve detection in terms of compositions of neurons in different image model layers, TODO and \citet{nanda2023progress} has explained how transformers implement modular addition through training. These projects have shed light on neural network internals \citep{grokking_power} and motivated architectural changes to models \citep{hippo}, but all have required significant human ingenuity. To combat this, we present an attempt to automate the \textit{discovery phase} of these projects.

\subsection{Background}
\begin{itemize}
    \item One paragraph on path expansion, generalised to ~“subgraph expansion”.
    \begin{itemize}
        \item  Review of Transformer Circuits (and residual circuits).
        \item In software reverse engineering, practitioners often look at the subgraphs of important model behavior (link [https://www.mandiant.com/resources/blog/flare-ida-pro-script-series-simplifying-graphs-ida](https://www.mandiant.com/resources/blog/flare-ida-pro-script-series-simplifying-graphs-ida), ideally better source). There are many parallels between mechanistic interpretability and this field ([Olah](https://transformer-circuits.pub/2022/mech-interp-essay/index.html)) and so there is precedent for the idea of finding a computational subgraph.
    \end{itemize}
    \item One paragraph on ROME \citet{meng2022locating}, IOI \cite{wang2022interpretability} and ``causal scrubbing'' \cite{}.
    \begin{itemize}
        \item i.e that subgraphs/paths need to be tested by causally corrupting things.
    \end{itemize}
    \item Related work
    \begin{itemize}
        \item Our work builds off of the methods of previous interpretability works \cite{elhage2021mathematical vig2019multiscale, meng2022locating}). However, our work generalize these previous methods to implement a general-purpose automated approach to explaining internals. 
        \item Geiger et al.’s \cite{} several papers, though this work does not consider the architecture-specific details of transformers.
        \item \cite{vig2019multiscale} = abstract causality.
        \item CausaLM and expectations and do interventions.
    \end{itemize}
\end{itemize}
\begin{figure}
  \centering
  \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Beautiful pedagogical plot goes here.}
\end{figure}
\subsection{Contributions}
\begin{enumerate}
    \item Automatic Circuit DisCovery (ACDC), our novel algorithm (Section 2).
    \item Validation of ACDC against existing methods of finding subnetworks (Section 3).
    \item Exploration of the circuits the algorithm automatically recovers, from previous interpretability works (Section 4).
\end{enumerate}
\subsection{Our Work}
\begin{itemize}
        \item The subgraphs that are produced are immediately useful for the isolation of sparse subsets of the model that help perform tasks. For example, surveying these subgraphs can allow the high level structure of model internals to be quickly checked (signpost Appendix from Chris Mathwin that shows high-level token positions that matter can be found).
        \begin{itemize}
            \item Additionally, the algorithm is helpful for generating hypotheses that can then be manually tested - practitioners can use our work to prompt investigation into specific circuit components in greater detail
        \end{itemize}
        \item Our research finds that
        \begin{enumerate}
            \item we can reduce the number of edges in the graph by a factor of 1000 and retain as much as 80\% performance on particular tasks (Section 3 and 4).
            \item it is possible to accurately approximate the effect of removing several edges by assuming linearity (adding up the effects of removing each individual edge). This observation was made in \cite{vig2019visualizing} when heads were zero-ablated, and we extend this observation considerably (Appendix D).
        \end{enumerate}
        \item possibly add a paper-width figure of the three algorithm steps here?
\end{itemize}
